This Thing Called Fairness: Disciplinary Confusion Realizing a Value in Technology

The explosion in the use of software in important sociotechnical systems has renewed focus on the study of the way technical constructs reflect policies, norms, and human values. This effort requires the engagement of scholars and practitioners from many disciplines. And yet, these disciplines often conceptualize the operative values very differently while referring to them using the same vocabulary. The resulting conflation of ideas confuses discussions about values in technology at disciplinary boundaries. In the service of improving this situation, this paper examines the value of shared vocabularies, analytics, and other tools that facilitate conversations about values in light of these disciplinary specific conceptualizations, the role such tools play in furthering research and practice, outlines different conceptions of "fairness" deployed in discussions about computer systems, and provides an analytic tool for interdisciplinary discussions and collaborations around the concept of fairness. We use a case study of risk assessments in criminal justice applications to both motivate our effort--describing how conflation of different concepts under the banner of "fairness" led to unproductive confusion--and illustrate the value of the fairness analytic by demonstrating how the rigorous analysis it enables can assist in identifying key areas of theoretical, political, and practical misunderstanding or disagreement, and where desired support alignment or collaboration in the absence of consensus.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'noacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
		Font changes for SIGCHI table captions


Version 1.56    Bug fixes
		Added \flushbottom to two column formats (Philip Quinn)
		The final punctuation for the list of concepts
		is now period instead of semilcolon (Philip Quinn)
		New command \Description to describe images for visually
		impaired users.

Version 1.57    Change of \baselinestretch now produces an error
		Booktabs is now always loaded
		Added option `balance' to balance last page in two-column mode
		E-mail is no longer split in addresses
		New samples (Stephen Spencer)

==> sections/extratext.tex <==
%deleted from other files

\subsection{Looking beyond artifacts}
Going beyond the latent fissure over fairness between the legislature and the judge, fairness in the criminal justice system is both about substantive rules and procedures.
Concerns with the black box nature of the COMPAS tool reflect concerns about procedural fairness because the proprietary nature of the system limits access to information about the system's model of criminological risk.
The fairness of these limitations was challenged in the recent case of the State of Wisconsin vs.
Eric Loomis (881 N.W.2d 749 (Wis.
2016)).
Loomis's pre-sentencing investigation report contained a COMPAS assessment showing he was high risk for future crime and future violent crime, as well as scoring high on several of COMPAS's ``needs assessments'', which evaluate the extent to which an individual has needs that align with one of several ``criminogenic theories'' (for example, whether that individual has access to sufficient economic opportunity or requires treatment for substance addiction).\footnote{
For a description of the available scales, see~\citep{northpointe2012practitioners}.
} Despite having pleaded guilty to only a lesser two of out of the five criminal counts levied against him, Loomis was given a sentence on the higher end of the guidelines for his offenses.
At his sentencing hearing, the judge specifically called out his risk to the community as reflected by the COMPAS assessment.
Loomis challenged his sentence in a post-conviction relief motion, arguing that his inability to review COMPAS for accuracy violated his due process right to be sentenced exclusively on the basis of accurate information disclosed to him.\footnote{
This standard is articulated in Gardner v.
Florida, 430 U.S.
349 (1977).
} Loomis further argued that COMPAS constituted an illegal consideration of his gender in the creation of the sentence and that this violated his due process rights.\footnote{
Specifically, Loomis argued that consideration of gender ``at all'' during sentencing was forbidden by the state supreme court in State v.
Harris, 2010 WI 79, ¶3, 326 Wis.
2d 685, 786 N.W.2d 409.
} Wisconsin uses COMPAS differently for men and for women, which Loomis argued constitutes impermissible gender discrimination.\footnote{
Presumably, and per information in briefs from the State of Wisconsin, the difference in use lies in the choice of population to which the scores are normalized.
COMPAS consists of 41 ``scales'' which represent key factors that might lead an individual to engage in some type of crime.
The scores, ranging from 1-10, are decile ranks (a score of 1 corresponds to being in the lowest 10\% of scores for the population and scale tested, a score of 2 to the next, and so on up to a score of 10 which corresponds to the highest 10\% of scores for that scale).
Scores can be normalized (converted from a numeric score derived from an individual's responses to the relevant COMPAS assessment questions into the 1-10 decile rankings just described) using male or female subpopulations of a roughly 30,000 person national sample made up of offenders grouped into subpopulations of prison/parole, jail, and probation.
There is further a ``composite'' population for each gender, made up of a subsample of the original population in proportion to the actual fractions of those subpopulations in correctional systems nationally (which we observe is likely heavily weighted towards offenders on probation).
We will not remark here on the functional validity of applying these nationally scaled scores to local offender populations, except to say that Northpointe does offer its customers locally normalized scales and validity studies for purchase when they are available.
No such validation or local normalization was available to the State of Wisconsin.}
Because the COMPAS mechanism is proprietary, Loomis was not able to establish that his risk or needs assessments would have been different on the women's scale.
Loomis eventually appealed to the Wisconsin State Supreme Court, which found that responsibility for using the outputs of the COMPAS system vest entirely in the agency of trial judges determining sentences, effectively subordinating the accountability of the technical tool to accountability of the humans who control it \citep{hlr2017loomis}.
Yet this solution seems incomplete: some of the issues scholars have raised around COMPAS are related to the social, legal, and organizational structure by which it is put into place, for which the judges are neither causally nor morally responsible.
While it is difficult to describe COMPAS as fair on either quantitative grounds (e.g., because of known disparities in score distributions by race and gender) or qualitative grounds (e.g., because its abuse of ecological reasoning causes dignitary harm, though possibly less than is caused by a perfunctory hearing without the tool), COMPAS and other risk assessment instruments are often described as fair on narrow, procedural grounds.

The mechanisms by which COMPAS rates people for risk are proprietary and not available for public review.
While we can disclose known problems to the humans when they usev the tool, as the court in \textit{Loomis} demanded, it is not clear this will overcome their automation bias or that they will not become inured to the warnings, creating a situation where the tool is either useless and ignored or dispositive and illegal under the Loomis standard.
The impact of risk-recidivism tools on local populations is generally unstudied and the data which would facilitate this often are not readily available.
The veracity of the model on local populations is often also unstudied, meaning that the tool is likely to sway decision-makers away from the facts on the ground through a patina of trustworthiness.
Finally, criteria tinkering of the sort described by Christin interferes with the reproducibility of the scores and the fidelity of records to the real world---there is a gap between the perceived objectivity of the score and the reality that human subjectivity influences it and this gap leads to an accountability gap any time the score is used.
Transparency---in all its conceptions---is sorely lacking in this example.

The debate also puts the many definitions of \textit{accountability} on display, which we can use the lexicon to help surface.
As a component of the larger criminal justice system, COMPAS must be accountable in the contexts in which it is used.
But arrestees, convicted criminals awaiting sentencing, parolees and the public at large wonder to what extent the system is fair and \textit{to whom} its predictions and scores are accountable. The \textit{Loomis} case demonstrates that even heaviweight efforts to hold this system to account face tall hurdles.

This focus on access to the information and models being used to make decisions fits neatly in notions of procedural due process, yet in the research community studying values in computer systems, these issues would likely be positioned as issues of transparency or explanation, rather than of fairness.

Finally, at a meta-level, one might ask whether encapsulating a portion of critical criminal justice decision-making in a technical artifact that is acquired through procurement processes, rather than developed through policy processes, risks inappropriately privatizing policy.
Such private decision-making risks imposing rules on society in a way that does not comport with our understanding of fair processes for developing and applying policy.
Is it fair for trade secret protections to be provided to a technical system that impacts decisions made by the state about incarceration and bail? This may seem unfair for reasons of public policy that are not about the substantive or procedural fairness of the tool itself or its application in a particular case.
Rather, these concerns rest with the process of developing, overseeing, and using the tool.
The tool may be considered unfair because it cedes too much in the way of policy to the innards of a technical artifact with too little certainty that it comports with the logics of judges, the access needs of criminal defendants, and the openness of policy development demanded by democratic norms of governance.


The COMPAS debates serve as an example of the many ways fairness can be defined, analyzed, and operationalized within a sphere of human activity, a sociotechnical system, or a piece of technology.
It reveals the futility of assessing fairness abstractly, if one aims to deliver meaningful solutions in practice.
Narrow views of the intrinsic fairness of a tool in isolation (as considered by both ProPublica and Northpointe in their lively debate) may not tell the entire fairness story.


The COMPAS debate also reminds us that public concern with the opacity and inscrutability of machine learning systems is part of long history of concern with unaccountable bureaucracies, both public and private.
Many of the concerns with algorithmically driven systems extend to inscrutable power structures of all sorts, not just new technology.
Existing social science and legal scholarship exploring the inscrutability of machine learning systems belie this connection, interrogating sociotechnical systems rather than particular algorithms.
Algorithms in this sense are a new form of bureaucracy, or a new piece of the bureaucratic apparatus~\citep{cuellar2016cyberdelegation}, and scholars demand that electronic databases or algorithms be accountable and fair along multiple dimensions~\citep{barocas2016big, selbst2017disparate}.
Machine learning systems and the primacy of data-driven decision-making have renewed interest in making the characteristics of governance available to the governed.
This renewed interest is no doubt in part because of a general interest in technological innovation, but it also likely that the need to decide explicitly on values and specify behaviors to optimize for or measure ahead of time when automating has drawn attention to issues that are latent in human systems but difficult to tease out and see.
After all, because software is ultimately a technical artifact embodied in a machine, we can interrogate its behavior and hold it to a higher standard than a human bureaucrat~\citep{kroll2018fallacy}.

%%%%%%%%%%============================%%%%%%%%%%%%%%%
%%%% NOTE FROM NITIN: COMMENTING OUT THE OLD VERSION OF THE FAIRNESS IN MACHINE LEARNING SECTION FROM PRIOR TO THE REVISE AND RESUBMIT TO ADDRESS THE REVIEWERS CONCERNS THAT WE WEREN'T THOROUGH ENOUGH [BLOCKED OFF WITH THE \iffalse and \fi] command]
%%%%%%%%%%============================%%%%%%%%%%%%%%%
\iffalse
Recent attention to the use of machine learning in socially critical applications has focused research energies on the problems of fairness in machine learning and statistical models more generally~\cite{hardt2018fairml}.
Broadly, notions of fairness have fallen into two categories: \emph{individual fairness} (i.e., treating like cases alike)~\cite{dwork2012fairness}; and \emph{group fairness} (i.e., treating groups---often defined by legally protected attributes---in a way that is somehow equal or equitable, such as by matching various statistics across groups~\cite{mitchell2018mirror, narayanan2018twentyone, mitchell2018catalogue, hardt2016equality}.
Both ideas stand in contrast to an intuitive notion of ``fairness through blindness'', the idea that simply removing attributes on the basis of which one does not wish to make predictions from the data upon which models are built will eliminate its effect from the model.
Blindness fails for many reasons, notably because it does not in fact, on its own, remove the impact of the data being blinded, which may be \emph{redundantly encoded} in other factors. Indeed, in cases where the attribute one desires to suppress is socially constructed, it may not be meaningful without this proxy information~\cite{kohler2018eddie}.

Group fairness measures can hide intuitively unfair behavior or lower the utility of classification for all groups~\cite{corbett2018measure}.
To counter this, Kearns et al. suggested to protect not only known groups, but a large set of the possible subgroups of a population~\cite{kearns2017gerrymandering}.
By contrast, Lipton, Chouldechova, and McAuley have suggested that fixing problems of disparate impact may inherently require disparate treatment~\cite{lipton2017does}.
But it is likely the case that it is not possible to discover populations of interest in a way that satisfies a set of natural requirements~\cite{kleinberg2003impossibility}.
However, it is also the case that many desireable group fairness desiderata are not achievable simultaneously in practice~\cite{kleinberg2016inherent, chouldechova2017fair}.

Jacobs and Wallach have suggested that problems of fairness in machine learning come down to failure to attend to issues of measurement and construct validity in models~\cite{jacobs2018measurement}. \emph{Construct validity} is a literature from statistics that evaluates models not only based on their predictive capacity but on their structure~\cite{messick1987validity, quinn2010analyze}.

Kusner et al. have argued that fairness in machine learning model outputs can be understood counterfactually in terms of how the inputs can be modulated to achieve different outcomes~\cite{kusner2017counterfactual}.
This leads into the idea of strategically manipulating one's attributes in order to get the most desirable output from a model and the related question of how to build a model to resist such gaming~\cite{hardt2016strategic}.
Notably, strategic behavior may have disparate effects (as individuals may have disparate access to the instruments of manipulation)~\cite{hu2018disparate} or broader social losses~\cite{milli2018social}.
Economists have long noted that such strategic behavior can cause statistical relationships to break down and be arbitraged away through the phenomenon of \emph{Goodhart's law}~\cite{goodhart1984problems}.
\fi
%%%%%%%%%%============================%%%%%%%%%%%%%%%
%%%% END %%%
%%%%%%%%%%============================%%%%%%%%%%%%%%%

